Fast Tendermint: Speeding Up a Foundational Consensus Protocol

Tendermint is among the most widely studied and deployed Byzantine fault-tolerant (BFT) consensus protocols, owing in part to its native leader-rotation mechanism that subsumes complex view changes. Like most partially-synchronous BFT protocols, Tendermint tolerates $f < n/3$ Byzantine processes and decides in three communication steps. Motivated by the push for lower-latency blockchains, a recent line of work shows that consensus can be solved in two communication steps when $f < n/5$. We present Fast Tendermint, an adaptation of Tendermint to the $n > 5f$ setting that decides in two communication steps in the good case, while preserving Tendermint's leader-rotation structure. Fast Tendermint collapses Tendermint's prevote and precommit steps into a single voting step and merges the $locked$ and $valid$ state. We give proofs of agreement, validity, and termination, and a formal specification in Quint, a modern surface syntax for TLA+, used to model-check the protocol.

==> macros.tex <==
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{algorithm}
\usepackage[indLines=false]{algpseudocodex}
\usepackage{booktabs}
\usepackage{aliascnt}
\usepackage{breqn}

\makeatletter
\let\lemma\@undefined
\let\endlemma\@undefined
\let\c@lemma\@undefined
\newaliascnt{lemma}{theorem}
\theoremstyle{plain}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}

\let\corollary\@undefined
\let\endcorollary\@undefined
\let\c@corollary\@undefined
\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\makeatother

\makeatletter
\algblockdefx[Upon]{Upon}{EndUpon}[1]{%
    \algpx@startCodeCommand\algpx@startIndent\textbf{upon}\ #1\ \textbf{do}%
}{%
    \algpx@endIndent%
}
\pretocmd{\Upon}{\algpx@endCodeCommand}{}{}
\pretocmd{\EndUpon}{\algpx@endCodeCommand[1]}{}{}
\algtext*{EndUpon}
\pretocmd{\Statex}{\algpx@endCodeCommand}{}{}
% Right-justified \Comment tabs to \linewidth minus the measured width of the
% comment, which lands ~0.68pt past the text edge and reports every commented
% line as overfull.  Reserve that slack.  \Comment indirects through
% algorithmicx's language layer, so patch the command it points at.
\expandafter\patchcmd\csname ALG@cmd@\ALG@L @algorithmiccomment\endcsname
    {\dimexpr \linewidth - \algpx@tmpLen \relax}
    {\dimexpr \linewidth - \algpx@tmpLen - 1pt \relax}
    {}{\PackageWarning{macros}{Could not patch \noexpand\Comment justification}}
\makeatother

\algnewcommand\HalfStatex{\Statex\vspace{-0.4\baselineskip}}

\algnewcommand\algbroadcast{\textbf{broadcast}\xspace}
\algnewcommand\algfrom{\textbf{from}\xspace}
\algnewcommand\algwith{\textbf{with}\xspace}
\algnewcommand\algwhile{\textbf{while}\xspace}
\algnewcommand\algand{\textbf{AND}\xspace}
\algnewcommand\algor{\textbf{OR}\xspace}
\algnewcommand\algschedule{\textbf{schedule}\xspace}
\algnewcommand\algafter{\textbf{after}\xspace}
\algnewcommand\algcancel{\textbf{cancel}\xspace}

\newcommand{\li}[1]{\langle#1\rangle}
\newcommand{\assign}{\leftarrow}

\newcommand{\Proposal}{\mathsf{PROPOSAL}}
\newcommand{\Prevote}{\mathsf{PREVOTE}}
\newcommand{\Precommit}{\mathsf{PRECOMMIT}}

\newcommand{\coord}{\mathsf{proposer}}
\newcommand{\timeoutPropose}{\mathsf{timeoutPropose}}
\newcommand{\timeoutPrecommit}{\mathsf{timeoutPrecommit}}
\newcommand{\getValue}{\mathsf{getValue}}
\newcommand{\valid}{\mathsf{validate}}

\newcommand{\StartRound}{\textproc{StartRound}}
\newcommand{\OnTimeoutPropose}{\textproc{OnTimeoutPropose}}
\newcommand{\OnTimeoutPrecommit}{\textproc{OnTimeoutPrecommit}}

\newcommand{\nil}{nil}
\newcommand{\id}{id}
\newcommand{\propose}{propose}
\newcommand{\precommit}{precommit}

\newcommand{\otm}{Original Tendermint\xspace}
\newcommand{\ftm}{Fast Tendermint\xspace}
\newcommand{\fftm}{Faster Tendermint\xspace}

\newcommand{\freshProposalRule}{fresh-proposal rule\xspace}
\newcommand{\reProposalRule}{re-proposal rule\xspace}
\newcommand{\precommitQuorumRule}{quorum any rule\xspace}
\newcommand{\observationRule}{observation rule\xspace}
% \newcommand{\fftmObsRule}{observation2 rule\xspace}
\newcommand{\decisionRule}{decision rule\xspace}

\newcommand{\ff}[1]{\textcolor{blue}{#1}}

%% Highlights text changed since commit 0d76c4d.
%% \del marks text removed since then (struck through, in red).
%% Uncomment the renewcommand lines to turn the highlighting off.
\newcommand{\chg}[1]{\textcolor{orange!90!black}{#1}}
\newcommand{\del}[1]{\textcolor{red}{\st{#1}}}
%\renewcommand{\chg}[1]{#1}
%\renewcommand{\del}[1]{}

\newcommand{\daniel}[1]{\textcolor{purple}{\textbf{Daniel:} #1}}
\newcommand{\preston}[1]{\textcolor{violet}{\textbf{Preston:} #1}}

\newcommand{\myparagraph}[1]{\vspace{1ex} \noindent \textbf{#1}}

%% Uncomment to remove... comments :D
%\renewcommand{\daniel}[1]{}
%\renewcommand{\preston}[1]{}

